Learning Weighted Representations for Generalization Across Designs

Predictive models that generalize well under distributional shift are often desirable and sometimes crucial to building robust and reliable machine learning applications. We focus on distributional shift that arises in causal inference from observational data and in unsupervised domain adaptation. We pose both of these problems as prediction under a shift in design. Popular methods for overcoming distributional shift make unrealistic assumptions such as having a well-specified model or knowing the policy that gave rise to the observed data. Other methods are hindered by their need for a pre-specified metric for comparing observations, or by poor asymptotic properties. We devise a bound on the generalization error under design shift, incorporating both representation learning and sample re-weighting. Based on the bound, we propose an algorithmic framework that does not require any of the above assumptions and which is asymptotically consistent. We empirically study the new framework using two synthetic datasets, and demonstrate its effectiveness compared to previous methods.

==> tables.tex <==
% TABLE AND FIGURE
\begin{figure}
\CenterFloatBoxes
\begin{floatrow}
\ffigbox[0.4\textwidth]
  {\includegraphics[width=0.3\textwidth]{fig/weighting-ipm.png}}
  {\caption{A caption for a figure in a figure and a table side by side}\label{fig:test}}
\killfloatstyle
\ttabbox[0.55\textwidth]
  {\begin{tabular}{lcc}
    \hline
    & $\rmse(\hat{\tau})$ & $\hat{R}_\pi(f)$ \\
    \hline
    OLS & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    OLS-IPW & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    Caus.For & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    BART & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    BART & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    BART & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    \hline
    GCFR-IPW & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    GCFR-Free & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    GCFR & $x.xx \pm .xx$ & $x.xx \pm .xx$ \\
    \hline
  \end{tabular}
  }
  {\caption{Causal effect estimation on IHDP.}\label{tab:test}}
\end{floatrow}
\end{figure}


\begin{table}[t!]
  \centering
  \caption{Results and standard errors in Causal effect estimation.\label{tab:results}}
  \begin{tabular}{l|cc|cc|c|c}
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{\bf IHDP} & \multicolumn{2}{c}{\bf Twins} & \multicolumn{1}{c}{\bf Jobs} & {\bf Warfarin} \\
    \multicolumn{1}{c}{} & $\rmse(\hat{\tau})$ & $\hat{R}_\pi(f)$ & $\rmse(\hat{\tau})$ & $\hat{R}_\pi(f)$ & Pol. risk & Pol. risk  \\
    \hline
    Lin            & $2.3 \pm .11$ & $1.6 \pm .05$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $.23 \pm .02$ & $x.x \pm .xx$ \\
    Lin-IPW        & $2.4 \pm .11$ & $1.7 \pm .05$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ \\
    Causal Forests & $3.8 \pm .18$ & $2.2 \pm .08$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $.20 \pm .02$ & $x.x \pm .xx$ \\
    BART           & $2.3 \pm .10$ & $2.1 \pm .07$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $.25 \pm .02$ & $x.x \pm .xx$ \\
    CFRW           & $.76 \pm .02$ & $1.1 \pm .01$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $.21 \pm .01$ & $x.x \pm .xx$\\
    \hline
    %GCFR-IPW       & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ \\
    %GCFR-Free      & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ \\
    GCFR           & $.70 \pm .06$ & $1.1 \pm .01$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ & $x.x \pm .xx$ \\
  \end{tabular}
\end{table}


\iffalse
\begin{figure}[tbp!]
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{fig/weighting-ipm.png}
    \caption{\label{fig:weighting_ipm}}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
    \begin{table}
      \begin{tabular}{c|c}
        hej & hej
      \end{tabular}
    \end{table}
  \end{subfigure}
  \caption{\label{fig:ihdp} Yada yada}
\end{figure}
\fi

